Extracting Summary Knowledge Graphs from Long Documents

Knowledge graphs capture entities and relations from long documents and can facilitate reasoning in many downstream applications. Extracting compact knowledge graphs containing only salient entities and relations is important but challenging for understanding and summarizing long documents. We introduce a new text-to-graph task of predicting summarized knowledge graphs from long documents. We develop a dataset of 200k document/graph pairs using automatic and human annotations. We also develop strong baselines for this task based on graph learning and text summarization, and provide quantitative and qualitative studies of their effect.

==> content_files/eval-analysis.tex <==
We analyzed a handful of abstracts to better understand the different scoring criteria proposed for this task. 
The gold graphs was hand-annotated to identify the most important entities, eliminating some "generic" nodes (e.g. ``method''), non-essential "other scientific term" nodes, and occasional duplicated nodes. In some cases, we added entities that were not in the gold reference but were identified by one or more of the automatic algorithms and seemed appropriate.
Entities identified by the automatic algorithms were hand-aligned to the reduced gold set. 
For untyped entities, the recall is higher on the reduced set for G2G and Pagerank, suggesting that these algorithms may be better capturing the most salient entities. The errors in types often involved unclear cases.  Trends in precision on the reduced graph were consistent with the automatic scoring. 
What is not explicitly captured by the current scoring algorithm is that some of the aligned nodes merge too many entities, which in part explains the low relation scores together with the impact of missing/inserted entities. 

==> content_files/intro.tex <==
\section{Introduction}

%[r] Determining the most salient information in a long document is a difficult but important challenge. 
%\rik{Determining the most salient entities and key relationships between them is a difficult but important challenge in understanding long documents such as scientific papers.}
%Automatic summarization \citep{Liu2019BertSum, Yasunaga2019sci-sum} partially addresses this problem, but conflates salient information identification with the daunting task of discourse structuring (and in the abstractive case, text generation as well). 
%Unlike natural language summaries, knowledge graphs explicitly capture entity and relation information in a compact, structured, human-interpretable format that facilitates a variety of downstream uses \cite{bosselut-etal-2019-comet, koncel-kedziorski-etal-2019-text, Peters2019KnowledgeEC}.   


%Knowledge graphs are important for information representation by explicitly capturing entity and relation information in a compact, structured, human-interpretable format. Such inherent structures also facilitate the reasoning in performing a variety of downstream tasks \cite{bosselut-etal-2019-comet, koncel-kedziorski-etal-2019-text, Peters2019KnowledgeEC}. 

\el{Maybe we still want to have one or two sentences to introduce knowledge graphs and remind people how cool they are? I think if we start right from document level IE, reviews (if they are not from IE community) may get confused.}

%Extracting entities and relations is important but challenging in understanding long documents such as scientific papers.
Document-level information extraction addresses the problem of capturing relations across distant sentences \citep{Jain2020SciREXAC, Jia2019DocumentLevelNR}.
However, another important challenge is presenting the most salient information from among the hundreds or more entity mentions and relations present in longer or dense documents such as scientific texts. 
Knowledge graphs explicitly encode entity and relation information in a compact, structured, human-interpretable format, but constructing a knowledge graph representation of a long text without considering information salience results in unwieldy graphs dominated by redundant and trivial information. 
Such graphs are of limited utility to human analysts and downstream applications alike. 
%Therefore, determining the most salient entities and key relationships between them in a text is important. 


Automatic summarization \citep{Liu2019BertSum, Yasunaga2019sci-sum} partially addresses the problem of identifying salient information in a document, but conflates salient information identification with the daunting task of discourse structuring (and in the abstractive case, text generation as well \el{now i think what in this parenthesis appears to be a bit confusing, as people may not know extractive VS abstractive summaries}). 

%\rik{Move this to related work} Summarizing entities and relations directly could reduce extra burden on models to learn how to write, as well as reduce confounding language artifacts for clearer evaluation. In fact, an increasing number of recent work [CITE] have proposed to automatically evaluate summarization models by applying information extraction or question answering models [CITE] to match entities or relations between generated and reference summaries. These newly proposed measures are found to have much higher correlations with human judgements than standard measures.


In addition, summarized knowledge graphs from multiple documents can be naturally merged by collapsing shared entity nodes to bring even richer information, which avoids the difficulty of summarizing multiple documents altogether into one piece of coherent text \el{I don't think I wrote what I meant ...}. And such summarized structures can be more easily leveraged to facilitate downstream tasks.


%%%%

%Summarizing entities and relations directly could reduce confounding language artifacts for clearer evaluation, as well as reduce extra burden on models to learn how to write. 

%This formulation is not without its challenges. 
%Long documents often involve hundreds of entities, making it especially challenging to determine which are most salient. %\citep{Jain2020SciREXAC}.
%Further, important relationships between entities are often established over the course of several pages, a challenge for relation identification.% \citep{Jia2019DocumentLevelNR}.

In this work, we propose an alternative formulation that summarizes a document with a knowledge graph, supported by a dataset of 200k scientific document/graph pairs that integrates automatic and human annotations from existing knowledge resources in the scientific domain. %with detailed explanation in Section~\ref{section:task-and-data}. 
We also outline an evaluation paradigm that addresses the variation in textual representation of entities. \el{we might not wanna emphasize much about the variation or noise in evaluation ... Instead we could talk about the three dimensions we propose for evaluation?}
%between the abstract and full text. 

%The new task complements current trends in document-level information extraction which aim to capture relations across distant sentences \citep{Jain2020SciREXAC, Jia2019DocumentLevelNR} or to fill a pre-defined metadata table with entities \cite{Hou2019IdentificationOT}, but  
%our task encourages models to identify a richer set of entities and relations.
%than prior work.
%Our work is also similar to \cite{falke2017concept-map}, which provides a small corpus of concept map annotations from OpenIE tuples for summarizing sets of documents. In contrast, we choose a science-specific annotation scheme that provides a more structured target. 

We develop and investigate two competitive baselines based on text summarization and graph learning models, providing analysis of their tradeoffs,
%strengths and weaknesses, 
along with general challenges posed in the dataset.
%We further show that a graph-pruning model with access to the gold entities outperforms either approach, but 
%An important observation is that target summary graphs include many relations which are not identified in a document's full text by current techniques. \el{this could raise dataset validity issue. I think we should say something like cross-sentence relations are hard to identify.} 
Our hope is that this task and data will facilitate research into future models that can better capture salient entities and identify the most important relations from long documents.\footnote{Data and models available at URL REDACTED}



